Deep Learning for Surface Wave Identification in Distributed Acoustic Sensing Data

Moving loads such as cars and trains are very useful sources of seismic waves, which can be analyzed to retrieve information on the seismic velocity of subsurface materials using the techniques of ambient noise seismology. This information is valuable for a variety of applications such as geotechnical characterization of the near-surface, seismic hazard evaluation, and groundwater monitoring. However, for such processes to converge quickly, data segments with appropriate noise energy should be selected. Distributed Acoustic Sensing (DAS) is a novel sensing technique that enables acquisition of these data at very high spatial and temporal resolution for tens of kilometers. One major challenge when utilizing the DAS technology is the large volume of data that is produced, thereby presenting a significant Big Data challenge to find regions of useful energy. In this work, we present a highly scalable and efficient approach to process real, complex DAS data by integrating physics knowledge acquired during a data exploration phase followed by deep supervised learning to identify "useful" coherent surface waves generated by anthropogenic activity, a class of seismic waves that is abundant on these recordings and is useful for geophysical imaging. Data exploration and training were done on 130~Gigabytes (GB) of DAS measurements. Using parallel computing, we were able to do inference on an additional 170~GB of data (or the equivalent of 10 days' worth of recordings) in less than 30 minutes. Our method provides interpretable patterns describing the interaction of ground-based human activities with the buried sensors.

==> Makefile <==
###############################################################################
# the latex command is pdflatex
LATEX = pdflatex
# the bibtex command is biber -- specified in preamble.tex in this directory
BIBTEX = bibtex

###############################################################################
# the main latex file is iptf-ccgrid20.tex in this directory
MAIN = main

###############################################################################
# Assume all LaTeX files (*.tex) are in this level and all figures are in figs
# directory and all bibtex entries are at this level with .bib
TEXFILES = ${wildcard *.tex}
BIBFILES = ${wildcard *.bib}
FIGS = ${wildcard *.pdf}

###############################################################################
# default target
.DEFAULT_GOAL := $(MAIN).pdf
$(MAIN): $(MAIN).pdf
.PHONY: $(MAIN) clean realclean

###############################################################################
# run LATEX command to generate the main PDF file
$(MAIN).pdf $(MAIN).log: $(TEXFILES) $(FIGS) $(BIBFILES)
	${LATEX} $(MAIN)
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	${BIBTEX} $(MAIN); ${LATEX} $(MAIN); fi;
	@if [ `fgrep undefined $(MAIN).log | fgrep Citation - | wc -l` -gt 0 ]; then \
	${BIBTEX} $(MAIN); ${LATEX} $(MAIN); fi;
	@while [ `fgrep -i 'Rerun ' $(MAIN).log | fgrep LaTeX - | wc -l` -gt 0 ]; do \
        ${LATEX} $(MAIN); \
        done

###############################################################################
# basic sanity check
check: missingincludes badrefs badbibs

# Extract a list of missing smartinclude files
missingincludes: $(MAIN).log
	@(grep -i "smartinclude: warning:" $< | \
	  sed 's/smartinclude: WARNING: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== SMARTINCLUDE WARNINGS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check log for: 
# - Multiply defined labels
# - Undefined labels
# - Undefined citations
# - Undefined acronyms (no messages for multiply-defined acronyms)
badrefs: $(MAIN).log
	@(grep -i "latex warning:" $< |\
	  grep -v -i "there were multiply-defined labels" | \
	  grep "multiply defined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MULTIPLY-DEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "latex warning:" $< | \
	  grep -v -i "there were undefined references" | \
	  grep -i "reference" | grep -i "undefined" |\
	  sed 's/LaTeX Warning: //' > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED LABELS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "package acronym warning:" $< | \
	  grep -i "acronym" | grep -i "not defined" |\
	  sed 's/Package acronym Warning: //' |\
	  sort | uniq > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED ACRONYMS =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

# Check BibTeX log for:
# - missing .bib files
# - missing database entries
# - repeated entries
# - string name undefined
# - errors in entries ("I was expecting...")
badbibs: $(MAIN).log
	${BIBTEX} $(MAIN)
	@(grep -i "i couldn't open database file " $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB FILES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--i didn't find a database entry for" \
	  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== MISSING BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "repeated entry--"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== REPEATED BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "warning--string name" $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== UNDEFINED STRINGS IN BIB =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)
	@(grep -i "i was expecting"  $(MAIN).blg > make.tmp.$$$$ ;\
	if [ -s make.tmp.$$$$ ]; then \
	  echo -e "\n===== ERRORS IN BIB ENTRIES =====" ; \
	  cat make.tmp.$$$$; \
	fi; \
	$(RM) make.tmp.$$$$)

clean:
	-@find . \( -name '*.aux' -print \) -o \( -name '*.log' -print \) \
		-o \( -name '*.bbl' -print \) -o \( -name '*.blg' -print \) \
		-o \( -name '*.toc' -print \) -o \( -name '*.out' -print \) \
		-o \( -name '*.bcf' -print \) -o \( -name '*~' -print \) \
		-o \( -name '*.maf' -print \) -o \( -name '*.mtc*' -print \) | xargs $(RM)

###############################################################################
# WARNING: removes the main target
realclean: clean
	$(RM) $(MAIN).pdf*

